How well can we determine ages and chemical abundances from spectral fitting of integrated light spectra?

The pixel-to-pixel spectral fitting technique is often used in studies of stellar populations. It enables the user to infer several parameters from integrated light spectra such as ages and chemical abundances. In this paper, we examine the question of how the inferred parameters change with the choice of wavelength range used. We have employed two different libraries of integrated light spectra of globular clusters (GCs) from the literature and fitted them to stellar population models using the code Starlight. We performed tests using different regions of the spectra to infer reddening, ages, [Fe/H] and [alpha/Fe]. Comparing our results to age values obtained from isochrone fitting and chemical abundances from high resolution spectroscopy, we find that: (1) The inferred parameters change with the wavelength range used; (2) The method in general retrieves good reddening estimates, specially when a wider wavelength range is fitted; (3) The ideal spectral regions for determination of age, [Fe/H], and [alpha/Fe] are: 4170-5540A, 5280-7020A, and 4828-5364A, respectively; (4) The retrieved age values for old metal-poor objects can be several Gyr younger than those resulting from isochrone fitting. We conclude that, depending on the parameter of interest and the accuracy requirements, fitting the largest possible wavelength range may not necessarily be the best strategy.

==> online_only_material.tex <==
%%%%%%%%%%%%%%%%% APPENDICES %%%%%%%%%%%%%%%%%%%%%
\appendix
\newpage
\onecolumn

\section{Online-only Material}

\subsection{Compilation of literature values}

\begin{landscape}
%\thispagestyle{empty}

\begin{longtable}{llllcclcl}
%\advance\leftskip-2.5cm
%\fontsize{5}{8}\selectfont
\caption{Globular clusters present in the WAGGS database and the reference values for ages and chemical abundances. The symbol '*' indicates values that were not found in our search.}\\
%\begin{tabular}{lllllllll}
\hline
ID      & Galaxy & RA {[}$^o${]} & Dec {[}$^o${]} & {[}Fe/H{]} & {[}Mg/Fe{]} & Reference for abundances                                 & Age (Gyrs)   & Reference for age    \\
\hline 
\endfirsthead
\caption{continued.}\\
\hline
ID      & Galaxy & RA {[}$^o${]} & Dec {[}$^o${]} & {[}Fe/H{]} & {[}Mg/Fe{]} & Reference for abundances                                 & Age (Gyrs)   & Reference for age    \\
\hline
\endhead
\hline
\endfoot  

NGC0104 & MW     & 6.024      & -72.081     & -0.768  $\pm$    0.031         & 0.52    $\pm$     0.03           & \citet{2009AeA...505..139C}  & 12.75 $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC0121 & SMC    & 6.701      & -71.536     & -1.41   $\pm$    0.07          & *       $\pm$     *              & \citet{2004oee..sympE..29J}  & 10.5  $\pm$ 0.5    & \citet{2008AJ....135.1106G}                        \\
NGC0330 & SMC    & 14.074     & -72.463     & -0.82   $\pm$    0.11          & -0.1    $\pm$     0.18           & \citet{1999AeA...345..430H}  & 0.03  $\pm$ 0.002  & \citet{2002ApJ...579..275S}                        \\
NGC0361 & SMC    & 15.542     & -71.605     & -1.16   $\pm$    *             & *       $\pm$     *              & \citet{2005ApJS..161..304M}  & 6.8   $\pm$ 0.5    & \citet{1998AJ....116.2395M}                        \\
NGC0362 & MW     & 15.809     & -70.849     & -1.17   $\pm$    0.05          & 0.33    $\pm$     0.04           & \citet{2013yCat..35570138C}  & 11.5  $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC0416 & SMC    & 16.994     & -72.355     & -1.22   $\pm$    *             & *       $\pm$     *              & \citet{1538-3881-138-5-1403} & 6     $\pm$ 0.5    & \citet{2008AJ....136.1703G}                        \\
NGC0419 & SMC    & 17.072     & -72.883     & -0.77   $\pm$    *             & *       $\pm$     *              & \citet{1538-3881-138-5-1403} & 1.45  $\pm$ 0.05   & \citet{2014ApJ...797...35G}                        \\
Fornax3 & Fornax & 39.951     & -34.258     & -2.33   $\pm$    *             & *       $\pm$     *              & \citet{2012AeA...546A..53L}  & 12.3  $\pm$ 1.4    & \citet{2016AeA...590A..35D}                       \\
Fornax4 & Fornax & 40.032     & -34.536     & -1.42   $\pm$    *             & *       $\pm$     *              & \citet{2012AeA...546A..53L}  & 10.2  $\pm$ 1.2    & \citet{2016AeA...590A..35D}                       \\
Fornax5 & Fornax & 40.588     & -34.102     & -2.09   $\pm$    *             & *       $\pm$     *              & \citet{2012AeA...546A..53L}  & 11.5  $\pm$ 1.5    & \citet{2016AeA...590A..35D}                       \\
NGC1261 & MW     & 48.068     & -55.216     & -1.19   $\pm$    0.02          & 0.2     $\pm$     0.1            & \citet{2012AAS...21915205F}  & 11.5  $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC1786 & LMC    & 74.783     & -67.745     & -1.75   $\pm$    0.01          & 0.35    $\pm$     0.36           & \citet{2010ApJ...717..277M}  & 12.3  $\pm$ *      & \citet{2010AJ....139..878S}                        \\
NGC1783 & LMC    & 74.787     & -65.987     & -0.35   $\pm$    *             & *       $\pm$     *              & \citet{2008AJ....136..375M}  & 1.7   $\pm$ 0.05   & \citet{2014ApJ...797...35G}                        \\
NGC1846 & LMC    & 76.891     & -67.461     & -0.5    $\pm$    *             & *       $\pm$     *              & \citet{2006AJ....132.1630G}  & 1.7   $\pm$ 0.05   & \citet{2014ApJ...797...35G}                        \\
NGC1850 & LMC    & 77.186     & -68.762     & -0.4    $\pm$    *             & *       $\pm$     *              & \citet{2015AeA...575A..62N}  & 0.1   $\pm$ 0.01   & \citet{2015AeA...575A..62N}                       \\
NGC1856 & LMC    & 77.372     & -69.128     & -0.3    $\pm$    *             & *       $\pm$     *              & \citet{2013MNRAS.431L.122B}  & 0.3   $\pm$ 0.03   & \citet{2013MNRAS.431L.122B}                        \\
NGC1866 & LMC    & 78.413     & -65.466     & -0.27   $\pm$    0.04          & -0.27   $\pm$     0.14           & \citet{2012ApJ...746...29C}  & 0.2   $\pm$ 0.02   & \citet{2013MNRAS.431L.122B}                        \\
NGC1851 & MW     & 78.528     & -40.047     & -1.18   $\pm$    0.07          & 0.35    $\pm$     0.03           & \citet{2011AeA...533A..69C}  & 11    $\pm$ 0.5    & \citet{2014ApJ...785...21M}                        \\
NGC1868 & LMC    & 78.651     & -63.955     & -0.39   $\pm$    *             & *       $\pm$     *              & \citet{1991AJ....101..515O}  & 1.1   $\pm$ 0.1    & \citet{2007AeA...462..139K}                       \\
NGC1898 & LMC    & 79.177     & -69.656     & -1.35   $\pm$    0.05          & *       $\pm$     *              & \citet{2004oee..sympE..29J}  & 11.8  $\pm$ *      & \citet{doi:10.1111/j.1365-8711.1998.t01-1-01860.x} \\
NGC1916 & LMC    & 79.652     & -69.407     & -1.54   $\pm$    0.04          & 0.32    $\pm$     0.2            & \citet{2012ApJ...746...29C}  & 12.9  $\pm$ *      & \citet{2003MNRAS.338...85M}                        \\
NGC1904 & MW     & 81.046     & -24.525     & -1.579  $\pm$    0.069         & 0.28    $\pm$     0.06           & \citet{2009AeA...505..139C}  & 14    $\pm$ 1      & \citet{2003astro.ph.11443G}                        \\
NGC1978 & LMC    & 82.188     & -66.236     & -0.54   $\pm$    0.06          & -0.05   $\pm$     0.3            & \citet{2012ApJ...746...29C}  & 1.9   $\pm$ 0.1    & \citet{2007AJ....133.2053M}                        \\
NGC2004 & LMC    & 82.678     & -67.286     & -0.58   $\pm$    *             & *       $\pm$     *              & \citet{2015AeA...575A..62N}  & 0.02  $\pm$ 0.001  & \citet{2015AeA...575A..62N}                       \\
NGC2019 & LMC    & 82.986     & -70.160     & -1.67   $\pm$    0.03          & 0.17    $\pm$     0.17           & \citet{2012ApJ...746...29C}  & 12.5  $\pm$ *      & \citet{doi:10.1111/j.1365-8711.1998.t01-1-01860.x} \\
NGC2100 & LMC    & 85.538     & -69.212     & 0.03    $\pm$    0.08          & *       $\pm$     *              & \citet{2012ApJ...746...29C}  & 0.02  $\pm$ 0.001  & \citet{2015AeA...575A..62N}                       \\
NGC2136 & LMC    & 88.241     & -69.493     & -0.55   $\pm$    0.23          & *       $\pm$     *              & \citet{2000AeA...360..133D}  & 0.1   $\pm$ 0.01   & \citet{2015AeA...575A..62N}                       \\
NGC2808 & MW     & 138.013    & -64.864     & -1.151  $\pm$    0.05          & 0.2     $\pm$     0.25           & \citet{2009AeA...505..139C}  & 11.5  $\pm$ 0.75   & \citet{2014ApJ...785...21M}                        \\
NGC3201 & MW     & 154.403    & -46.412     & -1.512  $\pm$    0.075         & 0.34    $\pm$     0.04           & \citet{2009AeA...505..139C}  & 12    $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC4147 & MW     & 182.526    & 18.543      & -1.84   $\pm$    0.02          & 0.42    $\pm$     0.03           & \citet{2016MNRAS.460.2351V}  & 12.75 $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC4590 & MW     & 189.867    & -26.744     & -2.265  $\pm$    0.07          & 0.35    $\pm$     0.06           & \citet{2009AeA...505..139C}  & 13    $\pm$ 1      & \citet{2010ApJ...708..698D}                        \\
NGC4833 & MW     & 194.891    & -70.876     & -2.02   $\pm$    0.01          & 0.27    $\pm$     0.22           & \citet{2014AeA...564A..60C}  & 13    $\pm$ 1.25   & \citet{2010ApJ...708..698D}                        \\
NGC5024 & MW     & 198.230    & 18.168      & -2.07   $\pm$    0.07          & *       $\pm$     *              & \citet{2016ApJ...824....5B}  & 13.25 $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC5139 & MW     & 201.697    & -47.480     & -1.53   $\pm$    *             & *       $\pm$     *              & \citet{globclust}            & 11    $\pm$ *      & \citet{2007ApJ...663..296V}                        \\
NGC5272 & MW     & 205.548    & 28.377      & -1.39   $\pm$    0.08          & 0.4     $\pm$     0.12           & \citet{2005AJ....129..303C}  & 12.5  $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC5286 & MW     & 206.612    & -51.374     & -1.72   $\pm$    0.01          & *       $\pm$     *              & \citet{2015MNRAS.450..815M}  & 13    $\pm$ 1      & \citet{2010ApJ...708..698D}                        \\
NGC5634 & MW     & 217.405    & -5.976      & -1.867  $\pm$    0.05          & 0.519   $\pm$     0.035          & \citet{2017AeA...600A.118C}  & 13    $\pm$ *      & \citet{2006AeA...456.1085M}                       \\
NGC5694 & MW     & 219.901    & -26.539     & -1.93   $\pm$    0.11          & 0.15    $\pm$     0.03           & \citet{2006ApJ...646L.119L}  & 13.6  $\pm$ *      & \citet{2005AJ....130..116D}                        \\
NGC5824 & MW     & 225.994    & -33.068     & -2.38   $\pm$    0.02          & -0.2    $\pm$     0.06           & \citet{2016MNRAS.455.2417R}  & 13.4  $\pm$ 1      & \citet{2005AJ....130..116D}                        \\
NGC5904 & MW     & 229.638    & 2.081       & -1.34   $\pm$    0.064         & 0.41    $\pm$     0.07           & \citet{2009AeA...505..139C}  & 12.25 $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC5927 & MW     & 232.003    & -50.673     & -0.47   $\pm$    0.02          & 0.27    $\pm$     0.02           & \citet{2018MNRAS.474.4541M}  & 12.25 $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC5986 & MW     & 236.512    & -37.786     & -1.54   $\pm$    0.08          & 0.28    $\pm$     0.13           & \citet{2017ApJ...842...24J}  & 13.25 $\pm$ 1      & \citet{2010ApJ...708..698D}                        \\
NGC6093 & MW     & 244.260    & -22.976     & -1.79   $\pm$    0.02          & 0.45    $\pm$     0.1            & \citet{2015AeA...578A.116C}  & 13.5  $\pm$ 1      & \citet{2010ApJ...708..698D}                        \\
NGC6121 & MW     & 245.897    & -26.526     & -1.168  $\pm$    0.012         & 0.55    $\pm$     0.03           & \citet{2009AeA...505..139C}  & 12.5  $\pm$ 5      & \citet{2010ApJ...708..698D}                        \\
NGC6139 & MW     & 246.918    & -38.849     & -1.579  $\pm$    0.058         & 0.495   $\pm$     0.043          & \citet{2015AeA...583A..69B}  & 13.2  $\pm$ 1      & \citet{2004AeA...428...79S}                       \\
NGC6171 & MW     & 248.133    & -13.054     & -1.033  $\pm$    0.038         & 0.51    $\pm$     0.04           & \citet{2009AeA...505..139C}  & 12.75 $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6218 & MW     & 251.809    & -1.949      & -1.33   $\pm$    0.066         & 0.52    $\pm$     0.04           & \citet{2009AeA...505..139C}  & 13.25 $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6254 & MW     & 254.288    & -4.100      & -1.575  $\pm$    0.076         & 0.49    $\pm$     0.04           & \citet{2009AeA...505..139C}  & 13    $\pm$ 1.25   & \citet{2010ApJ...708..698D}                        \\
NGC6266 & MW     & 255.303    & -30.114     & -1.1    $\pm$    0.07          & 0.42    $\pm$     0.07           & \citet{2015ApJ...813...97L}  & 12.5  $\pm$ *      & \citet{2005AJ....130..116D}                        \\
NGC6273 & MW     & 255.657    & -26.268     & -1.74   $\pm$    *             & *       $\pm$     *              & \citet{globclust}            & 13.2  $\pm$ *      & \citet{2005AJ....130..116D}                        \\
NGC6284 & MW     & 256.119    & -24.765     & -1.26   $\pm$    *             & *       $\pm$     *              & \citet{globclust}            & 12    $\pm$ *      & \citet{2005AJ....130..116D}                        \\
NGC6293 & MW     & 257.542    & -26.582     & -1.99   $\pm$    0.01          & -0.04   $\pm$     0.22           & \citet{2002AJ....124.1511L}  & 13    $\pm$ *      & \citet{2006AeA...456.1085M}                       \\
NGC6304 & MW     & 258.634    & -29.462     & -0.45   $\pm$    *             & *       $\pm$     *              & \citet{globclust}            & 12.75 $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6316 & MW     & 259.155    & -28.140     & -0.45   $\pm$    *             & *       $\pm$     *              & \citet{globclust}            & 10    $\pm$ 2      & \citet{2004AeA...428...79S}                       \\
NGC6333 & MW     & 259.797    & -18.516     & -1.77   $\pm$    *             & *       $\pm$     *              & \citet{globclust}            & *     $\pm$ *      & * \\
NGC6342 & MW     & 260.292    & -19.587     & -0.597  $\pm$    0.02          & 0.375   $\pm$     0.01           & \citet{2005MNRAS.356.1276O}  & 12.5  $\pm$ *      & \citet{2005AJ....130..116D}                        \\
NGC6356 & MW     & 260.896    & -17.813     & -0.4     $\pm$   *             & *       $\pm$     *              & \citet{globclust}            & 12.8  $\pm$ *      & \citet{2006AeA...456.1085M}                       \\
NGC6352 & MW     & 261.371    & -48.422     & -0.54    $\pm$   0.16          & 0.46    $\pm$     0.01           & \citet{2009AeA...493..913F}  & 13    $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC6362 & MW     & 262.979    & -67.048     & -1.07    $\pm$   0.01          & 0.54    $\pm$     0.01           & \citet{2017MNRAS.468.1249M}  & 12.5  $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC6388 & MW     & 264.072    & -44.735     & -0.441   $\pm$   0.025         & 0.21    $\pm$     0.07           & \citet{2009AeA...505..139C}  & 11.75 $\pm$ 0.75   & \citet{2014ApJ...785...21M}                        \\
NGC6397 & MW     & 265.175    & -53.674     & -1.988   $\pm$   0.061         & 0.46    $\pm$     0.04           & \citet{2009AeA...505..139C}  & 13.5  $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC6440 & MW     & 267.220    & -20.360     & -0.539   $\pm$   0.062         & 0.332   $\pm$     0.033          & \citet{2008MNRAS.388.1419O}  & 10    $\pm$ 2      & \citet{2004AeA...428...79S}                       \\
NGC6441 & MW     & 267.554    & -37.051     & -0.43    $\pm$   0.05          & 0.34    $\pm$     0.09           & \citet{2009AeA...505..139C}  & 12    $\pm$ 1      & \citet{2014ApJ...785...21M}                        \\
NGC6522 & MW     & 270.892    & -30.034     & -0.94    $\pm$   0.16          & 0.23    $\pm$     0.1            & \citet{2014AeA...570A..76B}  & 13    $\pm$ *      & \citet{2009AeA...507..405B}                       \\
NGC6528 & MW     & 271.207    & -30.056     & -0.172   $\pm$   0.03          & 0.352   $\pm$     0.03           & \citet{2005MNRAS.356.1276O}  & 11    $\pm$ 1      & \citet{2014ApJ...782...50L}                        \\
NGC6541 & MW     & 272.010    & -43.715     & -1.76    $\pm$   0.04          & 0.34    $\pm$     0.01           & \citet{2002AJ....124.1511L}  & 13.25 $\pm$ 1      & \citet{2010ApJ...708..698D}                        \\
NGC6553 & MW     & 272.323    & -25.909     & -0.35    $\pm$   0.19          & 0.05    $\pm$     0.03           & \citet{2017ApJ...834..105C}  & 13    $\pm$ *      & \citet{1538-3881-121-5-2638}                       \\
NGC6569 & MW     & 273.412    & -31.827     & -0.79    $\pm$   0.02          & 0.5     $\pm$     0.06           & \citet{2011MNRAS.414.2690V}  & 10.9  $\pm$ 2      & \citet{2004AeA...428...79S}                       \\
NGC6584 & MW     & 274.657    & -52.216     & -1.5     $\pm$   *             & *       $\pm$     *              & \citet{1990PASP..102..235R}  & 12.25 $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6624 & MW     & 275.919    & -30.361     & -0.69    $\pm$   0.02          & 0.42    $\pm$     0.05           & \citet{2011MNRAS.414.2690V}  & 13    $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6637 & MW     & 277.846    & -32.348     & -0.77    $\pm$   0.02          & 0.28    $\pm$     0.17           & \citet{2007RMxAC..28..120L}  & 12.5  $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6652 & MW     & 278.940    & -32.991     & -0.81    $\pm$   *             & *       $\pm$     *              & \citet{globclust}            & 13.25 $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC6656 & MW     & 279.100    & -23.905     & -1.76    $\pm$   0.02          & 0.39    $\pm$     0.03           & \citet{2009AeA...505.1099M}  & 13.5  $\pm$ 1      & \citet{2014ApJ...785...21M}                        \\
NGC6681 & MW     & 280.803    & -32.292     & -1.65    $\pm$   0.04          & 0.52    $\pm$     0.05           & \citet{2017ApJ...846...23O}  & 13    $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6715 & MW     & 283.764    & -30.480     & -1.51    $\pm$   0.16          & 0.28    $\pm$     0.09           & \citet{2010AeA...520A..95C}  & 13.25 $\pm$ 0.75   & \citet{2014ApJ...785...21M}                        \\
NGC6717 & MW     & 283.775    & -22.701     & -1.26    $\pm$   *             & *       $\pm$     *              & \citet{globclust}            & 13    $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6723 & MW     & 284.888    & -36.632     & -0.98    $\pm$   0.08          & 0.23    $\pm$     0.1            & \citet{2016AeA...587A..95R}  & 12.75 $\pm$ 0.5    & \citet{2010ApJ...708..698D}                        \\
NGC6752 & MW     & 287.717    & -59.985     & -1.555   $\pm$   0.074         & 0.5     $\pm$     0.05           & \citet{2009AeA...505..139C}  & 12.5  $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6809 & MW     & 294.999    & -30.965     & -1.934   $\pm$   0.074         & 0.47    $\pm$     0.1            & \citet{2009AeA...505..139C}  & 13.5  $\pm$ 1      & \citet{2010ApJ...708..698D}                        \\
NGC6838 & MW     & 298.444    & 18.779      & -0.832   $\pm$   0.051         & 0.49    $\pm$     0.04           & \citet{2009AeA...505..139C}  & 12.5  $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC6864 & MW     & 301.520    & -21.921     & -1.16    $\pm$   0.07          & 0.27    $\pm$     0.1            & \citet{2013AeA...554A..81K}  & 12.4  $\pm$ 2      & \citet{2004AeA...428...79S}                       \\
NGC6934 & MW     & 308.547    & 7.404       & -1.47    $\pm$   *             & *       $\pm$     *              & \citet{globclust}            & 12    $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC7006 & MW     & 315.372    & 16.187      & -1.46    $\pm$   0.03          & 0.12    $\pm$     0.17           & \citet{2013MNRAS.434..358S}  & 12.25 $\pm$ 0.75   & \citet{2011ApJ...738...74D}                        \\
NGC7078 & MW     & 322.493    & 12.167      & -2.32    $\pm$   0.069         & 0.45    $\pm$     0.19           & \citet{2009AeA...505..139C}  & 13.25 $\pm$ 1      & \citet{2010ApJ...708..698D}                        \\
NGC7089 & MW     & 323.363    & -0.823      & -1.65    $\pm$   *             & *       $\pm$     *              & \citet{globclust}            & 12.75 $\pm$ 0.75   & \citet{2010ApJ...708..698D}                        \\
NGC7099 & MW     & 325.092    & -23.180     & -2.344   $\pm$   0.069         & 0.51    $\pm$     0.04           & \citet{2009AeA...505..139C}  & 13.25 $\pm$ 1      & \citet{2010ApJ...708..698D} \\
\label{ref_table_online} 
%\end{tabular}
\end{longtable}
\end{landscape}


\subsection{Observed radial velocities and SNR}

\begin{longtable}{lrr}
\caption{Radial velocities (calculated as described in Section \ref{sec_prepross}) and average signal-to-noise for each spectrum of the WAGGS library.}\\
\hline
Spectrum file & Radial velocity (km/s) & $\langle$SNR$\rangle$ \\
\hline 
\endfirsthead
\caption{continued.}\\
\hline
Spectrum file & Radial velocity (km/s) & $\langle$SNR$\rangle$ \\
\hline
\endhead
\hline
\endfoot  
Fornax3\_B7000\_2015-08-09 & 61.2 $\pm$ 2.0  &40 \\ 
Fornax4\_B7000\_2015-08-10 & 50.7 $\pm$ 0.5  &20 \\ 
Fornax5\_B7000\_2015-08-11 & 62.0 $\pm$ 1.6  &13 \\ 
NGC0104\_B7000\_2015-01-30 & -17.5 $\pm$ 0.5 &359 \\ 
NGC0121\_B7000\_2015-08-11 & 143.5 $\pm$ 0.5 &57 \\ 
NGC0330\_B7000\_2015-11-02 & 155.0 $\pm$ 4.4  &24 \\ 
NGC0361\_B7000\_2015-11-02 & 173.8 $\pm$ 0.9  &13 \\ 
NGC0362\_B7000\_2015-01-30 & 223.5 $\pm$ 0.4 &176 \\ 
NGC0416\_B7000\_2015-08-08 & 157.4 $\pm$ 0.6 &32 \\ 
NGC0419\_B7000\_2015-12-18 & 185.9 $\pm$ 1.1 &44 \\ 
NGC1261\_B7000\_2015-08-08 & 73.4 $\pm$ 0.7  &78 \\ 
NGC1783\_B7000\_2016-04-02 & 277.5 $\pm$ 0.8 &27 \\ 
NGC1786\_B7000\_2016-10-03 & 257.8 $\pm$ 1.6 &25 \\ 
NGC1846\_B7000\_2016-04-01 & 240.1 $\pm$ 1.6  &2 \\ 
NGC1846\_B7000\_2016-04-02 & 240.7 $\pm$ 0.7 &8 \\ 
NGC1850\_B7000\_2016-04-01 & 248.2 $\pm$ 4.2 &37 \\ 
NGC1851\_B7000\_2015-01-31 & 322.4 $\pm$ 0.5  &262 \\ 
NGC1856\_B7000\_2016-04-02 & 265.8 $\pm$ 3.9 &37 \\ 
NGC1866\_B7000\_2016-04-02 & 301.5 $\pm$ 3.0 &38 \\ 
NGC1868\_B7000\_2016-10-03 & 285.4 $\pm$ 3.0 &19 \\ 
NGC1898\_B7000\_2016-10-03 & 209.0 $\pm$ 0.8&11 \\ 
NGC1904\_B7000\_2015-01-30 & 205.4 $\pm$ 0.9&68 \\ 
NGC1916\_B7000\_2015-12-18 & 272.6 $\pm$ 1.4&45 \\ 
NGC1978\_B7000\_2016-10-03 & 290.1 $\pm$ 0.8&25 \\ 
NGC2004\_B7000\_2016-09-30 & 294.6 $\pm$ 2.8&11 \\ 
NGC2019\_B7000\_2016-09-30 & 265.8 $\pm$ 1.0&19 \\ 
NGC2100\_B7000\_2015-12-17 & 33.9  $\pm$ 4.3&21 \\ 
NGC2136\_B7000\_2016-10-03 & 269.1  $\pm$ 3.9&24 \\ 
NGC2808\_B7000\_2015-01-31 & 106.0 $\pm$ 0.4&271 \\ 
NGC2808\_B7000\_2015-07-10 & 104.8 $\pm$ 0.4&194 \\ 
NGC3201\_B7000\_2015-04-15 & 493.9 $\pm$ 0.5&76 \\ 
NGC4147\_B7000\_2015-01-30 & 182.5 $\pm$ 1.5&17 \\ 
NGC4590\_B7000\_2015-04-13 & -90.1 $\pm$ 2.0&73 \\ 
NGC4833\_B7000\_2015-01-30 & 203.1 $\pm$ 2.0&73 \\ 
NGC5024\_B7000\_2015-01-30 & -63.4 $\pm$ 1.2&60 \\ 
NGC5139\_B7000\_2015-04-13 & 231.4 $\pm$ 1.2&45 \\ 
NGC5272\_B7000\_2016-04-02 & -145.0 $\pm$ 0.8 &93 \\ 
NGC5286\_B7000\_2015-04-14 & 61.8 $\pm$ 0.9&75 \\ 
NGC5634\_B7000\_2015-08-10 & -17.9 $\pm$ 1.3&83 \\ 
NGC5694\_B7000\_2015-08-11 & -142.9 $\pm$ 1.3&107 \\ 
NGC5824\_B7000\_2016-04-01 & -25.5 $\pm$ 1.3&43 \\ 
NGC5904\_B7000\_2015-04-15 & 58.0 $\pm$ 0.7&119 \\ 
NGC5927\_B7000\_2015-01-31 & -105.0 $\pm$ 0.6&43 \\ 
NGC5986\_B7000\_2015-07-10 & 96.4 $\pm$ 0.6&61 \\ 
NGC6093\_B7000\_2015-04-14 & 15.0 $\pm$ 0.9&13 \\ 
NGC6121\_B7000\_2015-04-15 & 75.6 $\pm$ 0.6&36 \\ 
NGC6139\_B7000\_2015-08-11 & 21.4 $\pm$ 0.5&34 \\ 
NGC6171\_B7000\_2015-07-09 & -35.5 $\pm$ 0.4&74 \\ 
NGC6218\_B7000\_2015-07-09 & -48.2 $\pm$ 0.5&53 \\ 
NGC6254\_B7000\_2015-04-13 & 78.2 $\pm$ 0.6&49 \\ 
NGC6266\_B7000\_2015-08-09 & -74.1 $\pm$ 0.4&105 \\ 
NGC6273\_B7000\_2015-08-10 & 142.7 $\pm$ 0.7&72 \\ 
NGC6284\_B7000\_2016-04-01 & 29.5 $\pm$ 0.4&29 \\ 
NGC6284\_B7000\_2016-09-29 & 36.0 $\pm$ 0.9&24 \\ 
NGC6293\_B7000\_2015-08-11 & -141.0 $\pm$ 1.4&72 \\ 
NGC6304\_B7000\_2015-04-14 & -109.1 $\pm$ 0.6&13 \\ 
NGC6304\_B7000\_2015-08-08 & -105.4 $\pm$ 0.5&16 \\ 
NGC6316\_B7000\_2016-04-02 & 98.4 $\pm$ 0.6&41 \\ 
NGC6333\_B7000\_2016-04-02 & 315.3 $\pm$ 0.7&68 \\ 
NGC6342\_B7000\_2015-07-10 & 118.6 $\pm$ 0.5&17 \\ 
NGC6342\_B7000\_2015-08-10 & 119.5 $\pm$ 0.5&13 \\ 
NGC6352\_B7000\_2015-07-09 & -127.6 $\pm$ 0.5&27 \\ 
NGC6356\_B7000\_2016-04-01 & 49.2 $\pm$ 0.5&40 \\ 
NGC6362\_B7000\_2015-08-11 & -10.0 $\pm$ 0.8&67 \\ 
NGC6388\_B7000\_2015-04-13 & 83.1 $\pm$ 0.5&175 \\ 
NGC6397\_B7000\_2015-04-13 & 18.3 $\pm$ 3.5&81 \\ 
NGC6440\_B7000\_2016-10-03 & -71.0 $\pm$ 1.4&11 \\ 
NGC6441\_B7000\_2015-04-15 & 22.3 $\pm$ 0.6&120 \\ 
NGC6522\_B7000\_2016-04-02 & -9.9 $\pm$ 0.5&75 \\ 
NGC6528\_B7000\_2015-04-13 & 211.7 $\pm$ 0.6&12 \\ 
NGC6541\_B7000\_2015-04-14 & -163.8 $\pm$ 1.0&134 \\ 
NGC6553\_B7000\_2015-04-15 & 1.7 $\pm$ 0.8 &14 \\ 
NGC6569\_B7000\_2015-08-10 & -52.1 $\pm$ 0.5&35 \\ 
NGC6584\_B7000\_2015-08-08 & 262.4 $\pm$ 0.6&22 \\ 
NGC6624\_B7000\_2015-07-09 & 52.8 $\pm$ 0.4&67 \\ 
NGC6637\_B7000\_2015-07-09 & 46.6 $\pm$ 0.5&67 \\ 
NGC6652\_B7000\_2015-08-08 & -97.3 $\pm$ 0.5&27 \\ 
NGC6656\_B7000\_2015-07-09 & -142.8 $\pm$ 0.7&64 \\ 
NGC6681\_B7000\_2015-08-10 & 218.3 $\pm$ 0.9&56 \\ 
NGC6715\_B7000\_2015-07-09 & 144.4 $\pm$ 0.6&72 \\ 
NGC6717\_B7000\_2015-04-15 & 31.0 $\pm$ 0.5&24 \\ 
NGC6717\_B7000\_2016-04-01 & 31.0 $\pm$ 0.6&41 \\ 
NGC6723\_B7000\_2016-09-29 & -98.2 $\pm$ 0.7&40 \\ 
NGC6752\_B7000\_2015-04-14 & -24.7 $\pm$ 1.0&111 \\ 
NGC6809\_B7000\_2015-08-09 & 180.3 $\pm$ 1.9&114 \\ 
NGC6838\_B7000\_2015-08-08 & -29.9 $\pm$ 0.6&39 \\ 
NGC6864\_B7000\_2015-08-10 & -187.2 $\pm$ 0.4&64 \\ 
NGC6934\_B7000\_2015-08-08 & -405.5 $\pm$ 1.0&19 \\ 
NGC7006\_B7000\_2015-08-09 & -380.3 $\pm$ 0.9&31 \\ 
NGC7078\_B7000\_2015-07-09 & -108.3 $\pm$ 2.0&105 \\ 
NGC7089\_B7000\_2015-07-09 & -3.3 $\pm$ 1.0&147 \\ 
NGC7099\_B7000\_2015-07-09 & -180.4 $\pm$ 2.9&16 \\ 
NGC7099\_B7000\_2016-09-30 & -190.1 $\pm$ 3.7&33 \\ 
NGC7099\_B7000\_2016-10-01 & -189.4 $\pm$ 4.5&66 \\ 
Fornax4\_R7000\_2015-08-10 & 46.6 $\pm$ 0.5  &32 \\ 
Fornax5\_R7000\_2015-08-11 & 71.9 $\pm$ 2.0  &12 \\ 
NGC0104\_R7000\_2015-01-30 & -15.9 $\pm$ 0.7  &727 \\ 
NGC0121\_R7000\_2015-08-11 & 144.9 $\pm$ 0.5  &97 \\ 
NGC0330\_R7000\_2015-11-02 & 154.9 $\pm$ 1.1  &61 \\ 
NGC0361\_R7000\_2015-11-02 & 168.7 $\pm$ 3.0  &34 \\ 
NGC0362\_R7000\_2015-01-30 & 222.1 $\pm$ 0.7  &306 \\ 
NGC0416\_R7000\_2015-08-08 & 155.9 $\pm$ 0.6  &55 \\ 
NGC0419\_R7000\_2015-12-18 & 201.1 $\pm$ 0.8  &71 \\ 
NGC1261\_R7000\_2015-08-08 & 71.4 $\pm$ 0.4  &149 \\ 
NGC1783\_R7000\_2016-04-02 & 279.2 $\pm$ 0.8  &43 \\ 
NGC1786\_R7000\_2016-10-03 & 259.1 $\pm$ 1.1  &42 \\ 
NGC1846\_R7000\_2016-04-02 & 241.3 $\pm$ 0.8  &17 \\ 
NGC1850\_R7000\_2016-04-01 & 244.6 $\pm$ 3.8  &66 \\ 
NGC1851\_R7000\_2015-01-31 & 321.9 $\pm$ 0.6  &379 \\ 
NGC1856\_R7000\_2016-04-02 & 265.4 $\pm$ 1.2  &58 \\ 
NGC1866\_R7000\_2016-04-02 & 301.8 $\pm$ 0.9  &47 \\ 
NGC1868\_R7000\_2016-10-03 & 284.6 $\pm$ 1.3  &22 \\ 
NGC1898\_R7000\_2016-10-03 & 208.1 $\pm$ 1.0  &20 \\ 
NGC1904\_R7000\_2015-01-30 & 204.2 $\pm$ 0.6  &109 \\ 
NGC1916\_R7000\_2015-12-18 & 297.8 $\pm$ 1.1  &71 \\ 
NGC1978\_R7000\_2016-10-03 & 292.0 $\pm$ 0.8  &24 \\ 
NGC2004\_R7000\_2016-09-30 & 307.4 $\pm$ 5.8  &1 \\ 
NGC2019\_R7000\_2016-09-30 & 277.1 $\pm$ 1.5  &11 \\ 
NGC2100\_R7000\_2015-12-17 & 253.4 $\pm$ 2.3  &24 \\ 
NGC2136\_R7000\_2016-10-03 & 269.9 $\pm$ 1.1  &23 \\ 
NGC2808\_R7000\_2015-01-31 & 107.3 $\pm$ 0.8  &474 \\ 
NGC2808\_R7000\_2015-07-09 & 104.4 $\pm$ 0.8  &244 \\ 
NGC3201\_R7000\_2015-01-31 & 496.9 $\pm$ 0.7  &163 \\ 
NGC3201\_R7000\_2015-04-15 & 496.8 $\pm$ 0.9  &188 \\ 
NGC4147\_R7000\_2015-01-30 & 181.8 $\pm$ 1.0  &32 \\ 
NGC4590\_R7000\_2015-04-13 & -96.9 $\pm$ 3.2  &176 \\ 
NGC4833\_R7000\_2015-01-30 & 203.0 $\pm$ 1.7  &90 \\ 
NGC5024\_R7000\_2015-01-30 & -63.1 $\pm$ 0.9  &102 \\ 
NGC5139\_R7000\_2015-04-13 & 233.9 $\pm$ 1.7  &63 \\ 
NGC5272\_R7000\_2016-04-02 & -142.6 $\pm$ 0.8  &133 \\ 
NGC5286\_R7000\_2015-04-14 & 62.3 $\pm$ 1.5  &180 \\ 
NGC5286\_R7000\_2016-04-01 & 59.8 $\pm$ 1.3  &64 \\ 
NGC5634\_R7000\_2015-08-10 & -14.0 $\pm$ 0.8  &158 \\ 
NGC5694\_R7000\_2015-08-11 & -137.5 $\pm$ 1.0  &169 \\ 
NGC5824\_R7000\_2016-04-01 & -22.0 $\pm$ 1.3  &19 \\ 
NGC5904\_R7000\_2015-04-15 & 57.7 $\pm$ 0.8  &189 \\ 
NGC5927\_R7000\_2015-01-31 & -105.4 $\pm$ 1.0  &117 \\ 
NGC5986\_R7000\_2015-07-10 & 97.1 $\pm$ 1.3  &116 \\ 
NGC6093\_R7000\_2015-04-14 & 10.9 $\pm$ 1.0  &60 \\ 
NGC6121\_R7000\_2015-04-15 & 74.9 $\pm$ 1.0  &76 \\ 
NGC6139\_R7000\_2015-08-11 & 22.3 $\pm$ 1.3  &111 \\ 
NGC6171\_R7000\_2015-07-09 & -31.6 $\pm$ 0.7  &134 \\ 
NGC6218\_R7000\_2015-07-09 & -40.9 $\pm$ 0.6  &102 \\ 
NGC6254\_R7000\_2015-04-13 & 70.5 $\pm$ 0.9  &125 \\ 
NGC6266\_R7000\_2015-08-09 & -73.4 $\pm$ 1.2  &298 \\ 
NGC6273\_R7000\_2015-08-10 & 143.2 $\pm$ 1.0  &159 \\ 
NGC6284\_R7000\_2016-09-29 & 22.7 $\pm$ 0.8  &67 \\ 
NGC6293\_R7000\_2015-08-11 & -141.9 $\pm$ 2.0  &142 \\ 
NGC6304\_R7000\_2015-04-14 & -108.2 $\pm$ 0.9  &65 \\ 
NGC6304\_R7000\_2015-08-08 & -100.2 $\pm$ 0.8  &85 \\ 
NGC6316\_R7000\_2016-04-02 & 100.4 $\pm$ 1.0  &117 \\ 
NGC6333\_R7000\_2016-04-02 & 313.9 $\pm$ 0.9  &111 \\ 
NGC6342\_R7000\_2015-08-10 & 120.6 $\pm$ 0.7  &133 \\ 
NGC6352\_R7000\_2015-07-09 & -125.2 $\pm$ 0.9  &60 \\ 
NGC6356\_R7000\_2016-04-01 & 47.4 $\pm$ 0.7  &89 \\ 
NGC6362\_R7000\_2015-08-11 & -8.4 $\pm$ 0.9  &143 \\ 
NGC6388\_R7000\_2015-04-13 & 80.8 $\pm$ 1.2  &281 \\ 
NGC6397\_R7000\_2015-04-13 & 12.2 $\pm$ 2.1  &111 \\ 
NGC6440\_R7000\_2016-10-03 & -61.2 $\pm$ 1.2  &68 \\ 
NGC6441\_R7000\_2015-04-15 & 10.0 $\pm$ 1.0  &285 \\ 
NGC6522\_R7000\_2016-04-02 & -10.1 $\pm$ 0.9  &172 \\ 
NGC6528\_R7000\_2015-04-13 & 210.5 $\pm$ 0.8  &34 \\ 
NGC6541\_R7000\_2015-04-14 & -163.4 $\pm$ 1.3  &245 \\ 
NGC6553\_R7000\_2015-04-15 & 2.2 $\pm$ 0.9  &61 \\ 
NGC6569\_R7000\_2015-08-10 & -45.8 $\pm$ 0.8  &92 \\ 
NGC6584\_R7000\_2015-08-08 & 259.2 $\pm$ 0.7  &69 \\ 
NGC6624\_R7000\_2015-07-09 & 50.7 $\pm$ 0.8  &142 \\ 
NGC6637\_R7000\_2015-07-09 & 43.4 $\pm$ 0.9  &131 \\ 
NGC6652\_R7000\_2015-08-08 & -91.0 $\pm$ 0.6  &90 \\ 
NGC6656\_R7000\_2015-07-09 & -142.8 $\pm$ 1.2  &137 \\ 
NGC6681\_R7000\_2015-08-10 & 219.9 $\pm$ 0.8  &104 \\ 
NGC6715\_R7000\_2015-07-09 & 142.8 $\pm$ 0.7  &233 \\ 
NGC6717\_R7000\_2016-04-01 & 26.6 $\pm$ 0.7  &107 \\ 
NGC6723\_R7000\_2015-07-10 & -96.2 $\pm$ 0.7  &138 \\ 
NGC6723\_R7000\_2016-04-01 & -95.9 $\pm$ 0.6  &47 \\ 
NGC6723\_R7000\_2016-09-29 & -95.4 $\pm$ 0.6  &75 \\ 
NGC6752\_R7000\_2015-04-14 & -26.3 $\pm$ 0.9  &91 \\ 
NGC6809\_R7000\_2015-08-09 & 171.8 $\pm$ 1.3  &175 \\ 
NGC6838\_R7000\_2015-08-08 & -24.2 $\pm$ 0.7  &192 \\ 
NGC6864\_R7000\_2015-08-10 & -188.7 $\pm$ 0.7  &144 \\ 
NGC6934\_R7000\_2015-08-08 & -407.6 $\pm$ 1.0  &89 \\ 
NGC7006\_R7000\_2015-08-09 & -383.3 $\pm$ 1.1  &138 \\ 
NGC7078\_R7000\_2015-07-09 & -101.8 $\pm$ 2.1  &323 \\ 
NGC7089\_R7000\_2015-07-09 & -3.5 $\pm$ 0.7  &240 \\ 
NGC7099\_R7000\_2015-07-09 & -182.0 $\pm$ 2.7  &27 \\ 
NGC7099\_R7000\_2016-09-30 & -187.2 $\pm$ 1.8  &135 \\ 
NGC7099\_R7000\_2016-10-01 & -186.1 $\pm$ 1.8  &102 \\ 
Fornax3\_U7000\_2015-08-09 & 64.2 $\pm$ 3.4  &9 \\ 
Fornax4\_U7000\_2015-08-10 & 45.6 $\pm$ 7.0  &4 \\ 
Fornax5\_U7000\_2015-08-11 & -  &2 \\ 
NGC0104\_U7000\_2015-01-30 & -14.8 $\pm$ 2.3  &74 \\ 
NGC0121\_U7000\_2015-08-11 & 145.5 $\pm$ 2.6  &10 \\ 
NGC0330\_U7000\_2015-11-02 & 164.2 $\pm$ 11.7  &16 \\ 
NGC0361\_U7000\_2015-11-02 & 171.1 $\pm$ 14.1  &4 \\ 
NGC0362\_U7000\_2015-01-30 & 223.0 $\pm$ 2.2  &28 \\ 
NGC0416\_U7000\_2015-08-08 & 156.7 $\pm$ 3.4  &6 \\ 
NGC0419\_U7000\_2015-12-18 & 196.9 $\pm$ 4.9  &8 \\ 
NGC1261\_U7000\_2015-08-08 & 73.1 $\pm$ 2.8  &19 \\ 
NGC1783\_U7000\_2016-04-02 & 279.2 $\pm$ 5.2  &5 \\ 
NGC1786\_U7000\_2016-10-03 & 258.8 $\pm$ 5.8  &5 \\ 
NGC1846\_U7000\_2016-04-02 & -  &1 \\ 
NGC1850\_U7000\_2016-04-01 & 255.9 $\pm$ 12.0  &16 \\ 
NGC1851\_U7000\_2015-01-31 & 321.4 $\pm$ 2.6  &45 \\ 
NGC1856\_U7000\_2016-04-02 & -  &12 \\ 
NGC1866\_U7000\_2016-04-02 & 306.5 $\pm$ 8.1  &9 \\ 
NGC1868\_U7000\_2016-10-03 & 277.6 $\pm$ 9.1  &3 \\ 
NGC1898\_U7000\_2016-10-03 & 211.4 $\pm$ 7.9  &2 \\ 
NGC1904\_U7000\_2015-01-30 & 205.6 $\pm$ 2.5  &13 \\ 
NGC1916\_U7000\_2015-12-18 & 284.8 $\pm$ 7.0  &8 \\ 
NGC1978\_U7000\_2016-10-03 & 284.4 $\pm$ 10.2  &2 \\ 
NGC2004\_U7000\_2016-09-30 & -  &0 \\ 
NGC2019\_U7000\_2016-09-30 & -  &1 \\ 
NGC2100\_U7000\_2015-12-17 & -  &11 \\ 
NGC2136\_U7000\_2016-10-03 & 267.1 $\pm$ 10.1  &4 \\ 
NGC2808\_U7000\_2015-01-31 & 106.0 $\pm$ 2.8  &45 \\ 
NGC2808\_U7000\_2015-07-09 & 102.7 $\pm$ 2.8  &19 \\ 
NGC3201\_U7000\_2015-01-31 & 497.7 $\pm$ 2.3  &11 \\ 
NGC3201\_U7000\_2015-04-15 & 500.7 $\pm$ 3.2  &14 \\ 
NGC4147\_U7000\_2015-01-30 & 184.0 $\pm$ 14.2  &4 \\ 
NGC4590\_U7000\_2015-04-13 & -98.1 $\pm$ 8.7  &29 \\ 
NGC4833\_U7000\_2015-01-30 & 200.6 $\pm$ 5.7  &8 \\ 
NGC5024\_U7000\_2015-01-30 & -62.9 $\pm$ 3.6  &11 \\ 
NGC5139\_U7000\_2015-04-13 & 234.0 $\pm$ 10.1  &6 \\ 
NGC5272\_U7000\_2016-04-02 & -144.4 $\pm$ 2.6  &6 \\ 
NGC5286\_U7000\_2015-04-14 & 64.6 $\pm$ 3.5  &17 \\ 
NGC5286\_U7000\_2016-04-01 & 60.9 $\pm$ 2.3  &6 \\ 
NGC5634\_U7000\_2015-08-10 & -15.1 $\pm$ 3.3  &20 \\ 
NGC5694\_U7000\_2015-08-11 & -141.5 $\pm$ 3.2  &20 \\ 
NGC5824\_U7000\_2016-04-01 & -26.6 $\pm$ 10.4  &2 \\ 
NGC5904\_U7000\_2015-04-15 & 56.3 $\pm$ 3.0  &23 \\ 
NGC5927\_U7000\_2015-01-31 & -104.8 $\pm$ 3.9  &4 \\ 
NGC5986\_U7000\_2015-07-10 & 97.6 $\pm$ 3.0  &10 \\ 
NGC6093\_U7000\_2015-04-14 & 14.3 $\pm$ 5.9  &6 \\ 
NGC6121\_U7000\_2015-04-15 & 73.2 $\pm$ 5.3  &6 \\ 
NGC6139\_U7000\_2015-08-11 & 23.5 $\pm$ 14.1  &4 \\ 
NGC6171\_U7000\_2015-07-09 & -39.8 $\pm$ 2.1  &8 \\ 
NGC6218\_U7000\_2015-07-09 & -42.1 $\pm$ 2.6  &8 \\ 
NGC6254\_U7000\_2015-04-13 & 65.1 $\pm$ 4.4  &11 \\ 
NGC6266\_U7000\_2015-08-09 & -77.4 $\pm$ 3.4  &19 \\ 
NGC6273\_U7000\_2015-08-10 & 142.5 $\pm$ 3.3  &10 \\ 
NGC6284\_U7000\_2016-09-29 & 25.4 $\pm$ 7.4  &4 \\ 
NGC6293\_U7000\_2015-08-11 & -142.2 $\pm$ 4.5  &11 \\ 
NGC6304\_U7000\_2015-04-14 & -109.3 $\pm$ 6.8  &3 \\ 
NGC6304\_U7000\_2015-08-08 & -97.9 $\pm$ 4.0  &4 \\ 
NGC6316\_U7000\_2016-04-02 & 99.7 $\pm$ 4.1  &4 \\ 
NGC6333\_U7000\_2016-04-02 & 315.6 $\pm$ 3.3  &7 \\ 
NGC6342\_U7000\_2015-08-10 & 122.7 $\pm$ 4.1  &6 \\ 
NGC6352\_U7000\_2015-07-09 & -124.9 $\pm$ 3.8  &3 \\ 
NGC6356\_U7000\_2016-04-01 & 49.6 $\pm$ 1.9  &5 \\ 
NGC6362\_U7000\_2015-08-11 & -11.6 $\pm$ 2.2  &10 \\ 
NGC6388\_U7000\_2015-04-13 & 81.6 $\pm$ 3.2  &17 \\ 
NGC6397\_U7000\_2015-04-13 & 22.9 $\pm$ 5.1  &18 \\ 
NGC6440\_U7000\_2016-10-03 & -  &1 \\ 
NGC6441\_U7000\_2015-04-15 & 14.8 $\pm$ 3.2  &15 \\ 
NGC6522\_U7000\_2016-04-02 & -9.6 $\pm$ 2.9  &8 \\ 
NGC6528\_U7000\_2015-04-13 & -  &1 \\ 
NGC6541\_U7000\_2015-04-14 & -163.9 $\pm$ 3.6  &31 \\ 
NGC6553\_U7000\_2015-04-15 & -  &1 \\ 
NGC6569\_U7000\_2015-08-10 & -46.3 $\pm$ 11.5  &3 \\ 
NGC6584\_U7000\_2015-08-08 & 260.7 $\pm$ 2.5  &6 \\ 
NGC6624\_U7000\_2015-07-09 & 52.7 $\pm$ 1.9  &8 \\ 
NGC6637\_U7000\_2015-07-09 & 43.9 $\pm$ 1.8  &9 \\ 
NGC6652\_U7000\_2015-08-08 & -96.3 $\pm$ 2.0  &7 \\ 
NGC6656\_U7000\_2015-07-09 & -144.8 $\pm$ 3.6  &10 \\ 
NGC6681\_U7000\_2015-08-10 & 217.6 $\pm$ 4.5  &11 \\ 
NGC6715\_U7000\_2015-07-09 & 142.1 $\pm$ 3.3  &25 \\ 
NGC6717\_U7000\_2016-04-01 & 28.4 $\pm$ 2.2  &8 \\ 
NGC6723\_U7000\_2015-07-10 & -97.9 $\pm$ 2.3  &13 \\ 
NGC6723\_U7000\_2016-04-01 & -97.7 $\pm$ 3.1  &4 \\ 
NGC6723\_U7000\_2016-09-29 & -98.4 $\pm$ 4.0  &7 \\ 
NGC6752\_U7000\_2015-04-14 & -27.2 $\pm$ 3.2  &11 \\ 
NGC6809\_U7000\_2015-08-09 & 168.3 $\pm$ 3.3  &27 \\ 
NGC6838\_U7000\_2015-08-08 & -19.3 $\pm$ 2.0  &10 \\ 
NGC6864\_U7000\_2015-08-10 & -191.0 $\pm$ 2.7  &11 \\ 
NGC6934\_U7000\_2015-08-08 & -404.6 $\pm$ 5.5  &6 \\ 
NGC7006\_U7000\_2015-08-09 & -382.8 $\pm$ 3.2  &14 \\ 
NGC7078\_U7000\_2015-07-09 & -104.1 $\pm$ 4.8  &43 \\ 
NGC7089\_U7000\_2015-07-09 & -4.1 $\pm$ 3.5  &33 \\ 
NGC7099\_U7000\_2015-07-09 & -187.1 $\pm$ 9.0  &4 \\ 
NGC7099\_U7000\_2016-09-30 & -187.7 $\pm$ 5.6  &21 \\ 
NGC7099\_U7000\_2016-10-01 & -189.6 $\pm$ 5.1  &15 \\ 

\label{vrad}
\end{longtable}

\newpage

\subsection{Resulting parameters from the fits performed with the $R_W$ range}

\begingroup
\footnotesize
\begin{longtable}{lrrrrrr}
\caption{Resulting parameters from the fits in $R_W$ and their uncertainties from the perturbed spectra of the WAGGS library.}\\
\hline
Spectrum & log($t_{light}$) & log($t_{mass}$) & $[Fe/H]_{light}$ & $[Fe/H]_{mass}$ & $[\alpha/Fe]_{light}$ & $[\alpha/Fe]_{mass}$ \\
\hline 
\endfirsthead
\caption{continued.}\\
\endhead
\hline
Spectrum & log($t_{light}$) & log($t_{mass}$) & $[Fe/H]_{light}$ & $[Fe/H]_{mass}$ & $[\alpha/Fe]_{light}$ & $[\alpha/Fe]_{mass}$ \\
\hline
\endhead
\hline
\endfoot  
Fornax3\_B7000\_2015-08-09 & 9.512$\pm$0.002 & 9.726$\pm$0.001 & -1.96$\pm$0.02 & -1.91$\pm$0.01 & 0.36$\pm$0.01 & 0.40$\pm$0.00 \\ 
Fornax4\_B7000\_2015-08-10 & 9.905$\pm$0.001 & 9.916$\pm$0.001 & -1.35$\pm$0.04 & -1.30$\pm$0.03 & 0.04$\pm$0.08 & 0.06$\pm$0.08 \\ 
Fornax5\_B7000\_2015-08-11 & 9.685$\pm$0.004 & 9.793$\pm$0.003 & -1.89$\pm$0.06 & -1.85$\pm$0.04 & 0.39$\pm$0.03 & 0.40$\pm$0.03 \\ 
NGC0104\_B7000\_2015-01-30 & 9.952$\pm$0.002 & 10.038$\pm$0.000 & -0.50$\pm$0.01 & -0.32$\pm$0.01 & 0.38$\pm$0.01 & 0.38$\pm$0.01 \\ 
NGC0121\_B7000\_2015-08-11 & 10.022$\pm$0.000 & 10.023$\pm$0.000 & -1.38$\pm$0.01 & -1.36$\pm$0.01 & 0.19$\pm$0.03 & 0.18$\pm$0.03 \\ 
NGC0330\_B7000\_2015-11-02 & 8.409$\pm$0.004 & 9.403$\pm$0.005 & -1.79$\pm$0.08 & -1.95$\pm$0.15 & 0.29$\pm$0.08 & 0.19$\pm$0.08 \\ 
NGC0361\_B7000\_2015-11-02 & 9.975$\pm$0.003 & 9.987$\pm$0.002 & -1.33$\pm$0.06 & -1.29$\pm$0.08 & 0.19$\pm$0.07 & 0.21$\pm$0.06 \\ 
NGC0362\_B7000\_2015-01-30 & 9.640$\pm$0.004 & 9.949$\pm$0.000 & -0.92$\pm$0.04 & -0.94$\pm$0.02 & 0.35$\pm$0.02 & 0.40$\pm$0.04 \\ 
NGC0416\_B7000\_2015-08-08 & 9.665$\pm$0.004 & 9.870$\pm$0.001 & -1.13$\pm$0.06 & -1.18$\pm$0.04 & 0.18$\pm$0.03 & 0.23$\pm$0.03 \\ 
NGC0419\_B7000\_2015-12-18 & 8.906$\pm$0.001 & 9.219$\pm$0.005 & -0.82$\pm$0.03 & -0.80$\pm$0.04 & 0.16$\pm$0.02 & 0.11$\pm$0.02 \\ 
NGC1261\_B7000\_2015-08-08 & 9.915$\pm$0.001 & 9.925$\pm$0.000 & -1.22$\pm$0.01 & -1.16$\pm$0.01 & 0.34$\pm$0.02 & 0.35$\pm$0.02 \\ 
NGC1783\_B7000\_2016-04-02 & 9.055$\pm$0.003 & 9.417$\pm$0.006 & -0.51$\pm$0.07 & -0.47$\pm$0.04 & 0.16$\pm$0.04 & 0.15$\pm$0.05 \\ 
NGC1786\_B7000\_2016-10-03 & 9.598$\pm$0.004 & 9.774$\pm$0.001 & -1.80$\pm$0.03 & -1.76$\pm$0.03 & 0.16$\pm$0.06 & 0.16$\pm$0.06 \\ 
NGC1846\_B7000\_2016-04-01 & 9.597$\pm$0.015 & 10.010$\pm$0.009 & -0.26$\pm$0.24 & -0.36$\pm$0.24 & 0.30$\pm$0.13 & 0.35$\pm$0.16 \\ 
NGC1846\_B7000\_2016-04-02 & 8.813$\pm$0.010 & 9.741$\pm$0.010 & -0.43$\pm$0.15 & -0.41$\pm$0.16 & 0.06$\pm$0.04 & 0.04$\pm$0.09 \\ 
NGC1850\_B7000\_2016-04-01 & 8.282$\pm$0.003 & 8.389$\pm$0.004 & -1.24$\pm$0.07 & -1.22$\pm$0.09 & 0.20$\pm$0.07 & 0.18$\pm$0.07 \\ 
NGC1851\_B7000\_2015-01-31 & 9.746$\pm$0.003 & 9.951$\pm$0.000 & -0.93$\pm$0.03 & -0.93$\pm$0.01 & 0.36$\pm$0.01 & 0.40$\pm$0.02 \\ 
NGC1856\_B7000\_2016-04-02 & 8.448$\pm$0.002 & 8.473$\pm$0.002 & -0.51$\pm$0.08 & -0.53$\pm$0.07 & 0.17$\pm$0.05 & 0.19$\pm$0.05 \\ 
NGC1866\_B7000\_2016-04-02 & 8.242$\pm$0.002 & 8.283$\pm$0.003 & -0.39$\pm$0.06 & -0.39$\pm$0.08 & 0.12$\pm$0.04 & 0.10$\pm$0.05 \\ 
NGC1868\_B7000\_2016-10-03 & 8.932$\pm$0.004 & 9.024$\pm$0.004 & -0.59$\pm$0.06 & -0.71$\pm$0.13 & 0.15$\pm$0.05 & 0.15$\pm$0.05 \\ 
NGC1898\_B7000\_2016-10-03 & 9.881$\pm$0.002 & 9.905$\pm$0.001 & -1.30$\pm$0.07 & -1.18$\pm$0.05 & 0.06$\pm$0.07 & 0.08$\pm$0.06 \\ 
NGC1904\_B7000\_2015-01-30 & 9.825$\pm$0.001 & 9.881$\pm$0.000 & -1.56$\pm$0.01 & -1.51$\pm$0.01 & 0.23$\pm$0.03 & 0.24$\pm$0.02 \\ 
NGC1916\_B7000\_2015-12-18 & 9.194$\pm$0.003 & 9.436$\pm$0.003 & -1.37$\pm$0.05 & -1.18$\pm$0.07 & 0.14$\pm$0.04 & 0.19$\pm$0.05 \\ 
NGC1978\_B7000\_2016-10-03 & 9.307$\pm$0.006 & 9.760$\pm$0.004 & -0.72$\pm$0.03 & -0.76$\pm$0.06 & 0.13$\pm$0.03 & 0.17$\pm$0.05 \\ 
NGC2004\_B7000\_2016-09-30 & 8.613$\pm$0.013 & 9.923$\pm$0.010 & -1.05$\pm$0.14 & -0.74$\pm$0.23 & 0.28$\pm$0.06 & 0.31$\pm$0.06 \\ 
NGC2019\_B7000\_2016-09-30 & 9.852$\pm$0.002 & 9.861$\pm$0.001 & -1.41$\pm$0.03 & -1.41$\pm$0.04 & 0.12$\pm$0.05 & 0.11$\pm$0.06 \\ 
NGC2100\_B7000\_2015-12-17 & 8.490$\pm$0.004 & 9.451$\pm$0.003 & -2.16$\pm$0.04 & -2.01$\pm$0.04 & 0.24$\pm$0.07 & 0.37$\pm$0.02 \\ 
NGC2136\_B7000\_2016-10-03 & 8.277$\pm$0.005 & 8.711$\pm$0.008 & -0.55$\pm$0.10 & -0.69$\pm$0.15 & 0.02$\pm$0.05 & 0.02$\pm$0.07 \\ 
NGC2808\_B7000\_2015-01-31 & 9.730$\pm$0.004 & 9.929$\pm$0.000 & -0.90$\pm$0.02 & -0.94$\pm$0.01 & 0.34$\pm$0.01 & 0.36$\pm$0.02 \\ 
NGC2808\_B7000\_2015-07-10 & 9.668$\pm$0.003 & 9.922$\pm$0.000 & -0.99$\pm$0.05 & -0.95$\pm$0.01 & 0.25$\pm$0.01 & 0.25$\pm$0.01 \\ 
NGC3201\_B7000\_2015-04-15 & 9.728$\pm$0.003 & 9.937$\pm$0.001 & -1.23$\pm$0.02 & -1.23$\pm$0.03 & 0.27$\pm$0.02 & 0.31$\pm$0.02 \\ 
NGC4147\_B7000\_2015-01-30 & 9.468$\pm$0.005 & 9.704$\pm$0.004 & -1.66$\pm$0.07 & -1.70$\pm$0.06 & 0.35$\pm$0.06 & 0.36$\pm$0.06 \\ 
NGC4590\_B7000\_2015-04-13 & 9.834$\pm$0.001 & 9.844$\pm$0.000 & -1.91$\pm$0.01 & -1.88$\pm$0.01 & 0.40$\pm$0.00 & 0.40$\pm$0.00 \\ 
NGC4833\_B7000\_2015-01-30 & 9.353$\pm$0.001 & 9.673$\pm$0.002 & -1.78$\pm$0.03 & -1.81$\pm$0.01 & 0.40$\pm$0.01 & 0.40$\pm$0.00 \\ 
NGC5024\_B7000\_2015-01-30 & 9.907$\pm$0.002 & 9.924$\pm$0.002 & -1.80$\pm$0.02 & -1.77$\pm$0.05 & 0.32$\pm$0.03 & 0.30$\pm$0.03 \\ 
NGC5139\_B7000\_2015-04-13 & 9.952$\pm$0.001 & 9.962$\pm$0.001 & -1.50$\pm$0.02 & -1.47$\pm$0.05 & 0.40$\pm$0.00 & 0.40$\pm$0.00 \\ 
NGC5272\_B7000\_2016-04-02 & 9.892$\pm$0.001 & 9.908$\pm$0.001 & -1.43$\pm$0.01 & -1.36$\pm$0.02 & 0.24$\pm$0.01 & 0.27$\pm$0.01 \\ 
NGC5286\_B7000\_2015-04-14 & 9.929$\pm$0.001 & 9.939$\pm$0.001 & -1.51$\pm$0.01 & -1.46$\pm$0.02 & 0.33$\pm$0.02 & 0.33$\pm$0.02 \\ 
NGC5634\_B7000\_2015-08-10 & 9.710$\pm$0.001 & 9.835$\pm$0.000 & -1.59$\pm$0.01 & -1.59$\pm$0.01 & 0.33$\pm$0.01 & 0.33$\pm$0.01 \\ 
NGC5694\_B7000\_2015-08-11 & 9.731$\pm$0.001 & 9.801$\pm$0.000 & -1.80$\pm$0.01 & -1.79$\pm$0.00 & 0.26$\pm$0.01 & 0.26$\pm$0.01 \\ 
NGC5824\_B7000\_2016-04-01 & 9.856$\pm$0.001 & 9.857$\pm$0.001 & -1.79$\pm$0.02 & -1.79$\pm$0.02 & 0.32$\pm$0.03 & 0.33$\pm$0.03 \\ 
NGC5904\_B7000\_2015-04-15 & 9.706$\pm$0.002 & 9.929$\pm$0.000 & -1.15$\pm$0.02 & -1.10$\pm$0.02 & 0.36$\pm$0.01 & 0.40$\pm$0.01 \\ 
NGC5927\_B7000\_2015-01-31 & 10.098$\pm$0.000 & 10.106$\pm$0.000 & -0.14$\pm$0.01 & -0.06$\pm$0.01 & 0.28$\pm$0.01 & 0.31$\pm$0.01 \\ 
NGC5986\_B7000\_2015-07-10 & 9.817$\pm$0.002 & 9.884$\pm$0.000 & -1.38$\pm$0.01 & -1.37$\pm$0.01 & 0.29$\pm$0.02 & 0.29$\pm$0.01 \\ 
NGC6093\_B7000\_2015-04-14 & 9.860$\pm$0.006 & 9.962$\pm$0.003 & -1.61$\pm$0.05 & -1.59$\pm$0.07 & 0.32$\pm$0.07 & 0.34$\pm$0.06 \\ 
NGC6121\_B7000\_2015-04-15 & 9.906$\pm$0.003 & 9.944$\pm$0.002 & -1.14$\pm$0.02 & -1.13$\pm$0.05 & 0.39$\pm$0.00 & 0.40$\pm$0.00 \\ 
NGC6139\_B7000\_2015-08-11 & 10.016$\pm$0.002 & 10.028$\pm$0.001 & -1.35$\pm$0.02 & -1.30$\pm$0.05 & 0.40$\pm$0.01 & 0.40$\pm$0.00 \\ 
NGC6171\_B7000\_2015-07-09 & 10.030$\pm$0.000 & 10.042$\pm$0.000 & -0.70$\pm$0.01 & -0.63$\pm$0.01 & 0.40$\pm$0.00 & 0.40$\pm$0.00 \\ 
NGC6218\_B7000\_2015-07-09 & 9.607$\pm$0.004 & 9.820$\pm$0.002 & -1.00$\pm$0.02 & -0.97$\pm$0.03 & 0.37$\pm$0.02 & 0.40$\pm$0.00 \\ 
NGC6254\_B7000\_2015-04-13 & 9.940$\pm$0.001 & 9.955$\pm$0.001 & -1.38$\pm$0.02 & -1.34$\pm$0.03 & 0.38$\pm$0.03 & 0.38$\pm$0.02 \\ 
NGC6266\_B7000\_2015-08-09 & 9.955$\pm$0.002 & 9.955$\pm$0.000 & -0.88$\pm$0.01 & -0.87$\pm$0.01 & 0.38$\pm$0.01 & 0.38$\pm$0.01 \\ 
NGC6273\_B7000\_2015-08-10 & 9.913$\pm$0.001 & 9.919$\pm$0.001 & -1.43$\pm$0.02 & -1.36$\pm$0.03 & 0.38$\pm$0.02 & 0.38$\pm$0.02 \\ 
NGC6284\_B7000\_2016-04-01 & 9.972$\pm$0.002 & 9.979$\pm$0.001 & -1.02$\pm$0.03 & -0.95$\pm$0.03 & 0.40$\pm$0.02 & 0.40$\pm$0.02 \\ 
NGC6284\_B7000\_2016-09-29 & 9.838$\pm$0.002 & 9.857$\pm$0.002 & -1.07$\pm$0.04 & -0.89$\pm$0.06 & 0.40$\pm$0.01 & 0.40$\pm$0.02 \\ 
NGC6293\_B7000\_2015-08-11 & 9.674$\pm$0.002 & 9.769$\pm$0.000 & -1.84$\pm$0.01 & -1.82$\pm$0.01 & 0.40$\pm$0.01 & 0.40$\pm$0.00 \\ 
NGC6304\_B7000\_2015-04-14 & 10.064$\pm$0.001 & 10.082$\pm$0.001 & -0.31$\pm$0.03 & -0.09$\pm$0.04 & 0.34$\pm$0.03 & 0.34$\pm$0.02 \\ 
NGC6304\_B7000\_2015-08-08 & 10.105$\pm$0.001 & 10.106$\pm$0.001 & -0.19$\pm$0.01 & -0.12$\pm$0.03 & 0.31$\pm$0.01 & 0.32$\pm$0.01 \\ 
NGC6316\_B7000\_2016-04-02 & 10.057$\pm$0.000 & 10.067$\pm$0.000 & -0.43$\pm$0.01 & -0.30$\pm$0.02 & 0.39$\pm$0.01 & 0.39$\pm$0.01 \\ 
NGC6333\_B7000\_2016-04-02 & 9.943$\pm$0.001 & 9.956$\pm$0.001 & -1.62$\pm$0.01 & -1.59$\pm$0.02 & 0.27$\pm$0.02 & 0.27$\pm$0.02 \\ 
NGC6342\_B7000\_2015-07-10 & 10.031$\pm$0.001 & 10.041$\pm$0.001 & -0.49$\pm$0.02 & -0.35$\pm$0.04 & 0.37$\pm$0.01 & 0.35$\pm$0.02 \\ 
NGC6342\_B7000\_2015-08-10 & 9.953$\pm$0.001 & 9.954$\pm$0.001 & -0.48$\pm$0.03 & -0.33$\pm$0.05 & 0.39$\pm$0.02 & 0.37$\pm$0.02 \\ 
NGC6352\_B7000\_2015-07-09 & 10.072$\pm$0.000 & 10.091$\pm$0.000 & -0.33$\pm$0.04 & -0.15$\pm$0.03 & 0.34$\pm$0.03 & 0.32$\pm$0.02 \\ 
NGC6356\_B7000\_2016-04-01 & 10.066$\pm$0.000 & 10.085$\pm$0.000 & -0.38$\pm$0.01 & -0.21$\pm$0.02 & 0.38$\pm$0.01 & 0.35$\pm$0.01 \\ 
NGC6362\_B7000\_2015-08-11 & 10.104$\pm$0.003 & 10.127$\pm$0.000 & -0.48$\pm$0.03 & -0.39$\pm$0.02 & 0.40$\pm$0.02 & 0.40$\pm$0.01 \\ 
NGC6388\_B7000\_2015-04-13 & 9.944$\pm$0.002 & 9.969$\pm$0.000 & -0.47$\pm$0.01 & -0.44$\pm$0.01 & 0.18$\pm$0.01 & 0.18$\pm$0.01 \\ 
NGC6397\_B7000\_2015-04-13 & 9.203$\pm$0.001 & 9.435$\pm$0.001 & -1.96$\pm$0.03 & -1.97$\pm$0.02 & 0.40$\pm$0.01 & 0.40$\pm$0.00 \\ 
NGC6440\_B7000\_2016-10-03 & 10.122$\pm$0.001 & 10.124$\pm$0.001 & -0.23$\pm$0.04 & -0.13$\pm$0.04 & 0.34$\pm$0.03 & 0.31$\pm$0.03 \\ 
NGC6441\_B7000\_2015-04-15 & 10.033$\pm$0.002 & 10.041$\pm$0.000 & -0.38$\pm$0.01 & -0.23$\pm$0.01 & 0.29$\pm$0.01 & 0.28$\pm$0.01 \\ 
NGC6522\_B7000\_2016-04-02 & 9.866$\pm$0.001 & 9.974$\pm$0.001 & -1.06$\pm$0.01 & -0.95$\pm$0.03 & 0.40$\pm$0.01 & 0.40$\pm$0.00 \\ 
NGC6528\_B7000\_2015-04-13 & 10.099$\pm$0.002 & 10.103$\pm$0.002 & 0.05$\pm$0.03 & 0.10$\pm$0.03 & 0.13$\pm$0.02 & 0.15$\pm$0.02 \\ 
NGC6541\_B7000\_2015-04-14 & 9.866$\pm$0.002 & 9.906$\pm$0.000 & -1.65$\pm$0.01 & -1.60$\pm$0.01 & 0.33$\pm$0.01 & 0.33$\pm$0.01 \\ 
NGC6553\_B7000\_2015-04-15 & 10.126$\pm$0.001 & 10.127$\pm$0.001 & 0.01$\pm$0.02 & 0.06$\pm$0.02 & 0.22$\pm$0.03 & 0.23$\pm$0.02 \\ 
NGC6569\_B7000\_2015-08-10 & 10.042$\pm$0.000 & 10.047$\pm$0.000 & -0.66$\pm$0.02 & -0.57$\pm$0.03 & 0.38$\pm$0.01 & 0.39$\pm$0.01 \\ 
NGC6584\_B7000\_2015-08-08 & 9.905$\pm$0.002 & 9.921$\pm$0.001 & -1.21$\pm$0.03 & -1.13$\pm$0.04 & 0.34$\pm$0.05 & 0.36$\pm$0.05 \\ 
NGC6624\_B7000\_2015-07-09 & 10.099$\pm$0.000 & 10.103$\pm$0.000 & -0.39$\pm$0.01 & -0.37$\pm$0.01 & 0.37$\pm$0.01 & 0.37$\pm$0.00 \\ 
NGC6637\_B7000\_2015-07-09 & 9.966$\pm$0.001 & 10.040$\pm$0.000 & -0.41$\pm$0.01 & -0.38$\pm$0.01 & 0.40$\pm$0.00 & 0.40$\pm$0.00 \\ 
NGC6652\_B7000\_2015-08-08 & 9.930$\pm$0.001 & 9.922$\pm$0.001 & -0.65$\pm$0.01 & -0.60$\pm$0.03 & 0.40$\pm$0.01 & 0.40$\pm$0.01 \\ 
NGC6656\_B7000\_2015-07-09 & 9.830$\pm$0.002 & 9.858$\pm$0.001 & -1.54$\pm$0.02 & -1.54$\pm$0.02 & 0.27$\pm$0.02 & 0.26$\pm$0.03 \\ 
NGC6681\_B7000\_2015-08-10 & 9.805$\pm$0.002 & 9.870$\pm$0.000 & -1.46$\pm$0.02 & -1.42$\pm$0.03 & 0.37$\pm$0.02 & 0.37$\pm$0.02 \\ 
NGC6715\_B7000\_2015-07-09 & 9.748$\pm$0.002 & 9.908$\pm$0.000 & -1.13$\pm$0.03 & -1.05$\pm$0.03 & 0.17$\pm$0.02 & 0.16$\pm$0.01 \\ 
NGC6717\_B7000\_2015-04-15 & 9.321$\pm$0.009 & 10.013$\pm$0.001 & -0.79$\pm$0.06 & -0.56$\pm$0.06 & 0.29$\pm$0.04 & 0.35$\pm$0.04 \\ 
NGC6717\_B7000\_2016-04-01 & 9.613$\pm$0.007 & 10.114$\pm$0.000 & -0.87$\pm$0.05 & -0.68$\pm$0.04 & 0.27$\pm$0.04 & 0.33$\pm$0.05 \\ 
NGC6723\_B7000\_2016-09-29 & 9.987$\pm$0.001 & 10.004$\pm$0.001 & -0.82$\pm$0.01 & -0.68$\pm$0.03 & 0.40$\pm$0.00 & 0.40$\pm$0.00 \\ 
NGC6752\_B7000\_2015-04-14 & 9.889$\pm$0.001 & 9.899$\pm$0.000 & -1.49$\pm$0.00 & -1.42$\pm$0.01 & 0.34$\pm$0.01 & 0.35$\pm$0.01 \\ 
NGC6809\_B7000\_2015-08-09 & 9.665$\pm$0.001 & 9.822$\pm$0.001 & -1.82$\pm$0.01 & -1.79$\pm$0.00 & 0.37$\pm$0.01 & 0.40$\pm$0.00 \\ 
NGC6838\_B7000\_2015-08-08 & 9.917$\pm$0.001 & 9.979$\pm$0.001 & -0.62$\pm$0.02 & -0.49$\pm$0.02 & 0.40$\pm$0.00 & 0.40$\pm$0.01 \\ 
NGC6864\_B7000\_2015-08-10 & 9.879$\pm$0.001 & 9.941$\pm$0.000 & -0.93$\pm$0.01 & -0.94$\pm$0.01 & 0.26$\pm$0.01 & 0.27$\pm$0.01 \\ 
NGC6934\_B7000\_2015-08-08 & 9.809$\pm$0.005 & 9.880$\pm$0.003 & -1.39$\pm$0.03 & -1.38$\pm$0.05 & 0.32$\pm$0.05 & 0.30$\pm$0.06 \\ 
NGC7006\_B7000\_2015-08-09 & 9.894$\pm$0.001 & 9.909$\pm$0.002 & -1.45$\pm$0.03 & -1.37$\pm$0.04 & 0.39$\pm$0.03 & 0.39$\pm$0.02 \\ 
NGC7078\_B7000\_2015-07-09 & 9.383$\pm$0.002 & 9.705$\pm$0.000 & -1.95$\pm$0.01 & -1.89$\pm$0.01 & 0.38$\pm$0.01 & 0.40$\pm$0.00 \\ 
NGC7089\_B7000\_2015-07-09 & 9.756$\pm$0.001 & 9.838$\pm$0.000 & -1.57$\pm$0.01 & -1.51$\pm$0.01 & 0.21$\pm$0.01 & 0.24$\pm$0.01 \\ 
NGC7099\_B7000\_2015-07-09 & 9.215$\pm$0.005 & 9.541$\pm$0.004 & -1.90$\pm$0.06 & -1.90$\pm$0.06 & 0.36$\pm$0.03 & 0.39$\pm$0.01 \\ 
NGC7099\_B7000\_2016-09-30 & 9.175$\pm$0.002 & 9.427$\pm$0.002 & -1.94$\pm$0.04 & -1.94$\pm$0.03 & 0.37$\pm$0.04 & 0.39$\pm$0.02 \\ 
NGC7099\_B7000\_2016-10-01 & 9.225$\pm$0.001 & 9.478$\pm$0.001 & -1.97$\pm$0.01 & -1.95$\pm$0.02 & 0.40$\pm$0.01 & 0.40$\pm$0.00
\label{incertezas_perturb}
\end{longtable}
\endgroup


%\section{Observed radial velocities obtained from \sc{Starlight}}
%\begin{figure}
	% To include a figure from a file named example.*
	% Allowable file formats are eps or ps if compiling using latex
	% or pdf, png, jpg if compiling using pdflatex
%	\includegraphics[width=\columnwidth]{figures/plot_v0.png}
%   \caption{Radial velocities by \textsc{Starlight} against the reference values.}
%  \label{plot_v0}
%\end{figure}

%\pc{Adicionar uma tabela com os valores de velocidade radial que o Starlight obteve para os GCs}


%\section{Fit for all clusters}
%\begin{figure*}
%\onecolumn
%	\includegraphics[scale=0.28]{figures/plot_4828-5364.png}
%    \caption{Observed data from WAGGS (in black) and their respective synthetic spectra fitted by \textsc{Starlight} in the $R_W$ range (in red).}
%    \label{res1}
%\end{figure*}




%If you want to present additional material which would interrupt the flow of the main paper,
%it can be placed in an Appendix which appears after the list of references.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


